Characterization of Fully Coupled FBSDE in Terms of Portfolio Optimization

We provide a verification and characterization result of optimal maximal sub-solutions of BSDEs in terms of fully coupled forward backward stochastic differential equations. We illustrate the application thereof in utility optimization with random endowment under probability and discounting uncertainty. We show with explicit examples how to quantify the costs of incompleteness when using utility indifference pricing, as well as a way to find optimal solutions for recursive utilities.

==> chap05.tex <==
\section{Dual Representation and Existence of Optimal Solutions}\label{sec:05}

Let $(\hat{\pi}, X, Y,Z)$ be an optimal solution of the optimization problem, and we assume that $\partial_{y}g=\partial_x g$ as well as $\partial_{\hat{z}}g=\partial_{\hat{r}}g$.
Assume furthermore that
\begin{equation*}
    Y_t=F-\int_{t}^{T}\left(b Y+cZ+\hat{c}\cdot \hat{\pi}+b X-g^{\ast}(\hat{c}, b,b,c) \right)ds -\int_{}^{} Z \cdot dW
\end{equation*}
where $(\hat{c}, b,b,c)=\partial g(\hat{\pi},X,Y,Z)$.
We define $\pi^\ast=\pi^\ast(X,y,z,u,v)$ such that
\begin{equation*}
    \partial_{y}g(\pi^\ast,X, y,z)=u \quad \text{and}\quad \partial_{z}g(\pi^\ast,X,y,z)=v
\end{equation*}
It follows that
\begin{equation*}
    \partial g(\pi^\ast(X, Y, Z, b,c), X, Y, Z)=\left( c,b,b,c \right)=\partial g(\pi, X, Y, Z)
\end{equation*}


Suppose that there exists a point-wise solution $\hat{\pi}^\ast(y,z, u, v)$ of
\begin{equation*}
    \begin{cases}
        X^\ast(y,z,u,v)&=\displaystyle x+\int_{0}^{t}\hat{\pi}^\ast(y,z,u,v) \cdot d\hat{W} \\
        \\
        (\hat{v}, u, u, v) & = \partial g(\hat{\pi}^\ast, X^\ast, y,z)=\partial g(\hat{\pi},X,y,z)
    \end{cases}
\end{equation*}
It follows that 
\begin{equation*}
    \begin{cases}
        \hat{\pi}^\ast&:=\hat{\pi}^\ast(Y,Z,\partial_{y}g(\hat{\pi},X,Y,Z), \partial_{z}g(\hat{\pi},X,Y,Z))\\
        \\
        X^\ast &:=\displaystyle X^\ast(Y,Z,\partial_{y}g(\hat{\pi},X,Y,Z), \partial_{z}g(\hat{\pi},X,Y,Z))=x+\int_{}^{} \hat{\pi}^\ast \cdot d\hat{W}
    \end{cases}
\end{equation*}
satisfies
\begin{equation}\label{eq:gradient}
    \partial g(\pi^\ast, X^\ast, Y,Z)=\partial g(\hat{\pi},X,Y,Z)=\left( \hat{c}, b,b,c \right)
\end{equation}
Let us show that $(Y,Z)$ satisfies 
\begin{equation*}
    Y_s\leq Y_t-\int_{s}^{t} g\left( \hat{\pi}^\ast, X^\ast, Y,Z \right)ds-\int_{s}^{t}Z \cdot dW 
\end{equation*}
By means of \eqref{eq:gradient}, it follows that
\begin{align*}
    g(\pi,X,Y,Z) & \geq \langle (\hat{c},b,b,c),(\hat{\pi},X,Y,Z)-( \hat{\pi}^\ast, X^\ast, Y,Z )\rangle +g(\hat{\pi}^\ast,X^\ast,Y,Z)\\
                 & = \hat{c}\cdot \left( \hat{\pi}-\hat{\pi}^\ast \right)+b(X - X^\ast)+g\left( \hat{\pi}^\ast, X^\ast,Y,Z \right)
\end{align*}
Since $(Y,Z)$ is maximal sub-solution it follows that
\begin{align*}
    Y_s & \leq Y_t-\int_{s}^{t}g\left(  \hat{\pi}, X,Y,Z \right)ds -\int_{s}^{t}Z\cdot d W\\
        & \leq Y_t - \int_{s}^{t} g\left( \hat{\pi}^\ast, X^\ast, Y,Z \right)ds-\int_{s}^{t}Z\cdot dW-\int_{s}^{t} \left( \hat{c}\cdot \left( \hat{\pi}-\hat{\pi}^\ast \right)+b(X - X^\ast)\right)ds
\end{align*}


\begin{theorem}
    It holds
    \begin{equation*}
        Y^\pi_0=\inf_{b \in \mathcal{D}, c \in bmo}\left\{ E\left[ M_T^{bc}F-\int_{0}^{T}M_t^{bc}\left( \hat{r}_t \pi_t +x_t\pi\bullet \tilde{W}_t-g_t^\ast(\hat{r}_t,x_t,b_t,c_t) \right)dt  \right] \right\}
    \end{equation*}
    where $r=\partial_{\tilde{z}}g(\pi,X^\pi,Y^\pi,Z^\pi)$ and $x=\partial_{x}g(\pi,X^\pi,Y^\pi,Z^\pi)$.

    Suppose that $\partial_r g=\partial_{\tilde{z}}$ and $\partial_x=\partial_y g$\footnote{As in the different financial case studies of the previous Section \ref{sec:03}.}, and there exists an optimal $\pi^\ast$ in $bmo$ such that $Y^{\pi^\ast}_0\geq Y^\pi_0$ for every $\pi$ in $bmo$.
    If $Y^\pi_0$ admits a gradient for every $\pi$, and there exists an optimal $\pi^\ast$, then the fully coupled forward backward stochastic differential equation \eqref{eq:sufficient} has a solution.
\end{theorem}
\begin{proof}
    We know that
    \begin{multline*}
        g(\pi_t,X^\pi_t,y,z)=\sup_{\tilde{r},x,b,c}\left\{ by+cz+\tilde{r} \pi_t+x X^\pi_t -g^\ast(\tilde{r},x,b,c)\right\}\\
        =\sup_{b,c}\left\{ by+cz+\hat{r}_t\pi_t+x_t X^\pi_t -g^\ast(r_t,x_t,b,c) \right\}\\
        =\sup_{b,c}\left\{ by+cz-h^\ast(b,c) \right\}
    \end{multline*}
    where
    \begin{equation*}
        \hat{r}_t=\tilde{r}_t(y,z)=\partial_{r}g_t(\pi_t,X^\pi_t,y,z), \quad \text{and}\quad x_t=x_t(y,z)=\partial_x g_t(\pi_t,X^\pi_t,y,z)
    \end{equation*}
    and
    \begin{equation*}
        h^\ast(b,c)=g^\ast_t(\tilde{r}_t,x_t, b,c)-\tilde{r}_t\pi_t-x_t X^\pi_t
    \end{equation*}
    According to \cite{DrapeauTangpi} adapted to forward dependent structure with the assumptions of \citep{mainberger2016}, as well as adaptation to the linear boundedness it follows that it holds
    \begin{equation*}
        Y^\pi_0=\inf_{b \in \mathcal{D}, c \in bmo}\left\{ E\left[ M_T^{bc}F-\int_{0}^{T}M_t^{bc}h^\ast_t(\pi_t,X^\pi_t,b_t,c_t)dt  \right] \right\}
    \end{equation*}

    Suppose that $\pi^\ast$ is an optimal solution and that in a neighborhood of $\pi^\ast$, every $Y^\pi_0$ admits a gradient $b^\pi$, $c^\pi$.
    In particular, it holds
    \begin{equation*}
        Y^\pi_t=F-\int_{t}^{T}\hat{c}^\pi_s \pi_s+b^\pi_s \pi\bullet \hat{W}_s+b^\pi_s Y^\pi_t+c_sZ^\pi_s ds-\int_{t}^{T}Z^\pi_s dW_s.
    \end{equation*}
    and therefore each maximal sub-solution in a neighborhood of $\pi^\ast$ is a solution itself.
    Using the notations $\Delta\pi=\pi-pi^\ast$, Optimality yields
    \begin{equation*}
        Y_0^\pi-Y^{\pi^\ast}_0 = -E\left[ \int_{0}^{T}M_t^{bc}\left(\hat{c}^\ast_t \Delta \pi_t + b_t\Delta \pi \bullet \hat{W}_t\right) dt\right]
    \end{equation*}
    
\end{proof}
\newpage

\begin{example}
    For incomplete marker, we consdier $h(y,z):=e^y+\dfrac{1}{2}\{|z_1|^2+|z_2|^2\}$. 
    By the arguments in Section 4, we need to solve the following FBSDE system
    \begin{equation*}
        \begin{cases}
            X_t=& x+\int_0^t\left(\theta^1_s+V^1_s-Z^1_s\right)dW^{\theta^1}_s, \\
            Y_t=&F-\int_t^T\left(e^{Y_s+X_s}+\frac{1}{2}(\theta^1_s+V^1_s)^2 +\frac{1}{2}(Z^2_s)^2-\left(\theta^1_s+V^1_s\right)\theta^1_s\right)ds\\
            &\quad\quad-\int_t^TZ^1_sdW^{\theta^1}_s-\int_t^TZ^2_sdW^2_s,\\
            U_t=&0-\int_t^T\left(e^{Y_s+X_s}+\frac{1}{2}(V^1_s)^2+\frac{1}{2}(V^2_s)^2\right)ds\\
            &-\int_t^TV^1_sdW^{\theta^1}_s-\int_t^TV^2_sdW^2_s,
        \end{cases}
    \end{equation*}
    It is equilvalent to solve
    \begin{equation}\label{FBSDE system-4}
        \begin{cases}
            X_t=& x+\int_0^t\left(\theta^1_s+V^1_s-Z^1_s\right)dW^{\theta^1}_s, \\
            Y_t=&F-\int_t^T\left(e^{Y_s+X_s}+\frac{1}{2}(\theta^1_s+V^1_s)^2 +\frac{1}{2}(Z^2_s)^2-\left(\theta^1_s+V^1_s\right)\theta^1_s \right)ds\\
            &\qquad\qquad-\int_t^TZ^1_sdW^{\theta^1}_s-\int_t^TZ^2_sdW^2_s,\\
            U_t=&0-\int_t^T\left(e^{Y_s+X_s}+\frac{1}{2}(V^1_s)^2-\frac{1}{2}(V^2_s)^2+V^2_sZ^2_s\right)ds\\
            &-\int_t^TV^1_sdW^{\theta^1}_s-\int_t^TV^2_sdW^2_s,
        \end{cases}
    \end{equation}
    we can give the solution to the FBSDE system (\ref{FBSDE system-4}) explicitly.
    \begin{enumerate}[label=\textit{Step \arabic*:}, fullwidth]
        \item     \begin{equation}\label{BSDE-examp 4.2-1}
                \hat{Y}_t=F-\int_t^T\left(\frac{1}{2}(\theta^1_s)^2+\frac{1}{2}\left(\hat{Z}^2_s\right)^2-\left(\theta^1_s+\hat{Z}^1_s\right)\theta^1_s\right)ds+\int_t^T\hat{Z}^1_sdW^1_s+\int_t^T\hat{Z}^2_sdW^2_u,
            \end{equation}
            admits a unique solution $(\hat{Y},\hat{Z}^1,\hat{Z}^2)\in\mathcal{S}^\infty\times  BMO\times BMO$.
            Indeed $\hat{Z}^2=0$.
        \item Define
            \begin{equation}\label{eqn-examp-4.2-2}
                X_t=x+\int_0^t\left(\theta^1_s+\hat{Z}^1_s\right)dW^{\theta^1}_s.
            \end{equation}
            Therefore, it holds
            \begin{equation*}
                X_T=x+\hat{Y}_0+\frac{1}{2}\int_{0}^{T}(\theta^1_t)^2+(\hat{Z}^2_t)^2dt+\int_0^T\theta^1_tdW^1_t-\int_0^T\hat{Z}^2_tdW^2_t.
            \end{equation*}
        \item Let
            \begin{equation*}
                \tilde{X}_t=x+\hat{Y}_0+\frac{1}{2}\int_{0}^{t}(\theta^1_s)^2+(\hat{Z}^2_s)^2ds+\int_0^t\theta^1_sdW^1_s-\int_0^t\hat{Z}^2_sdW^2_s.
            \end{equation*}
            Applying It\^{o}'s formula to $e^{-\tilde{X_t}}$, we obtain
            \begin{equation*}
                e^{-\tilde{X}_t}=e^{-X_T}+\int_t^{T}e^{-\tilde{X}_s}\theta^1_sdW^1_s-\int_t^{T}e^{-\tilde{X}_s}\hat{Z}^2_sdW^2_s.
            \end{equation*}
            Let
            \begin{align*}
                \begin{cases}
                    e^{-\tilde{Y}_t}&=e^{-\tilde{X}_t}+(T-t),\\
                    \tilde{Z}^1_t&=-\left(1-\frac{T-t}{e^{-\tilde{Y}_t}}\right)\theta^1_t,\\
                    \tilde{Z}^2_t&=\left(1-\frac{T-t}{e^{-\tilde{Y}_t}}\right)\hat{Z}^2_t.
                \end{cases}
            \end{align*}
            It is easy to check that
            \begin{equation*}
                e^{-\tilde{Y}_t}=e^{-X_T}+\{T-t\}+\int_t^Te^{-\tilde{Y}_s}\tilde{Z}^1_sdW^1_s+\int_t^Te^{-\tilde{Y}_s}\tilde{Z}^2_sdW^2_s.
            \end{equation*}
            Let
            \begin{equation*}
                \begin{cases}
                    Y_t&:=\tilde{Y}_t-X_t\\
                    U_t&:=\tilde{Y}_t-\hat{Y}_t-X_t,\\
                    V^1_t&:=\tilde{Z}^1_t-\theta^1_t,\\
                    Z^1_t&:=\tilde{Z}^1_t-\theta^1_t-\hat{Z}^1_t,\\
                    Z^2_t&:=\tilde{Z}^2_t,\\
                    V^2_t&:=\tilde{Z}^2_t+\hat{Z}^2_t.
                \end{cases}
            \end{equation*}
            Then $(X;Y,Z^1,Z^2;U,V^1,V^2)$ is the unique solution of FBSDE (\ref{FBSDE system-4}).

    \end{enumerate}
\end{example}



